Rethinking the Truly Unsupervised Image-to-Image Translation

Every recent image-to-image translation model inherently requires either image-level (i.e. input-output pairs) or set-level (i.e. domain labels) supervision. However, even set-level supervision can be a severe bottleneck for data collection in practice. In this paper, we tackle image-to-image translation in a fully unsupervised setting, i.e., neither paired images nor domain labels. To this end, we propose a truly unsupervised image-to-image translation model (TUNIT) that simultaneously learns to separate image domains and translates input images into the estimated domains. Experimental results show that our model achieves comparable or even better performance than the set-level supervised model trained with full labels, generalizes well on various datasets, and is robust against the choice of hyperparameters (e.g. the preset number of pseudo domains). Furthermore, TUNIT can be easily extended to semi-supervised learning with a few labeled data.

==> Truly unsupervised img2img (arXiv version)/0.abstract.tex <==
\begin{abstract}
Every recent image-to-image translation model inherently requires either image-level (\ie input-output pairs) or set-level (\ie domain labels) supervision. However, even set-level supervision can be a severe bottleneck for data collection in practice. In this paper, we tackle image-to-image translation in a fully unsupervised setting, \ie, neither paired images nor domain labels. To this end, we propose a truly unsupervised image-to-image translation model (TUNIT) that simultaneously learns to separate image domains and translates input images into the estimated domains. 
Experimental results show that our model achieves comparable or even better performance than the set-level supervised model trained with full labels, generalizes well on various datasets, and is robust against the choice of hyperparameters (\eg the preset number of pseudo domains). Furthermore, TUNIT can be easily extended to semi-supervised learning with a few labeled data. 
\end{abstract}


==> Truly unsupervised img2img (arXiv version)/1.introduction.tex <==
\section{Introduction}
\label{sec:introduction}
 Given an image of one domain, image-to-image translation is a task to generate the plausible images of the other domains. Based on the success of conditional generative models \cite{2014cGAN,2015cVAE}, many image translation methods have been proposed either using \emph{image-level} supervision (\eg paired data)~\cite{2017Pix2Pix,2017Cycada,2017bicyclegan,wang2018pix2pixhd,park2019spade} or using \emph{set-level} supervision (\eg domain labels) \cite{2017CycleGAN,2017DiscoGAN,2017UNIT,2018MUNIT,2019FUNIT,2020DRIT++}. 
Though the latter approach is generally called \emph{unsupervised} as a counterpart of the former, it actually assumes that the domain labels are given \textit{a priori}. This assumption can be a serious bottleneck in practice as the number of domains and samples increases. For example, labeling individual samples of a large dataset (\eg FFHQ) is expensive, and the distinction across domains can be vague.

We first clarify that unsupervised image-to-image translation should strictly denote the task \textit{without any supervision} neither paired images nor domain labels. Under this rigorous definition, our goal is to develop an unsupervised translation model given a mixed set of images of many domains (\Fref{fig:introduction}). We argue that the unsupervised translation model is valuable in three aspects. First of all, it significantly reduces the effort of data annotation for model training. As a natural byproduct, the unsupervised model can be robust against the noisy labels produced by the manual labeling process. More importantly, it serves as a strong baseline to develop the semi-supervised image translation models. To tackle this problem, we design our model having three sub-modules: 1) clustering the images by approximating the set-level characteristics (\ie domains), 2) encoding the individual content and style of an input image, respectively, and 3) learning a mapping function among the estimated domains. 

\figIntro

To this end, we introduce a \texttt{guiding network}. The guiding network consists of a shared encoder with two branches, where one provides pseudo domain labels and the other encodes images into feature vectors (style codes). We employ a differentiable clustering method based on mutual information maximization for estimating the domain labels and contrastive loss for extracting the style codes. The clustering helps the guiding network to group similar images into the same category. Meanwhile, the contrastive loss helps the model to understand the dissimilarity among images and learn better representations. We find that, by solving two tasks together within the same module, both benefit from each other. Specifically, the clustering can exploit rich representations learned by the contrastive loss and improve the accuracy of estimated domain labels. By taking advantage from the clustering module, the style code can also acknowledge the similarity within the same domain, thereby faithfully reflecting the domain-specific nature. 

For both more efficient training and effective learning, we jointly train the guiding network and GAN in an end-to-end manner. 
% our guiding network participates in the translation process as well. 
This allows the guiding network to understand the recipes of domain-separating attributes based on GAN's feedback, and the generator encourages the style code to contain rich information so as to fool the domain-specific discriminator. 
Thanks to these internal and external interactions of the guiding network and GAN, 
% between the guiding network and GAN, 
our model successfully separates domains and translates images; a truly unsupervised image-to-image translation. 

We quantitatively and qualitatively compare the proposed model with the existing set-level supervised models under unsupervised and semi-supervised settings. The experiments on various datasets show that the proposed model outperforms the baselines over all different levels of supervision. Our ablation study shows that the guiding network helps the image translation model to largely improve the performance. Our contributions are summarized as follows: 
\begin{itemize}[leftmargin=*]
\setlength\itemsep{0mm}
  \item We clarify the definition of unsupervised image-to-image translation and to the best of our knowledge, our model is the first to succeed in this task in an end-to-end manner.
  \item We propose the guiding network to handle the unsupervised translation task and show that the interaction between translation and clustering is helpful for the task.
  \item The quantitative and qualitative comparisons for the unsupervised translation task on four public datasets show the effectiveness of TUNIT, which clearly outperforms the previous arts.
  \item TUNIT is insensitive to the hyperparameter (\ie the number of clusters) and serves as a strong baseline for the semi-supervised setting-- TUNIT outperforms the current state-of-the-art semi-supervised image translation model.
\end{itemize}


%-- 이전 원본 --
% To this end, we introduce a \texttt{guiding network} that simultaneously solves unsupervised domain classification and style encoding. It has two branches of providing pseudo domain labels and encoding style features, which are later used in the discriminator and the generator training, respectively. We employ a differentiable clustering method that uses mutual information maximization for estimating domain labels. This helps the guiding network group similar images together while evenly separate their categories. For embedding style codes, we adopt a contrastive loss~\cite{2006contrastive,2019MoCo,2020simclr}, which leads the model to understand the dissimilarity among images, resulting in better representation learning. Finally, conditioned on the style features and domain labels from the guiding network, we use generative adversarial networks (GAN) to learn the image translation functions across domains. 
%-- 이전 원본 끝 --

% \jj{To this end, we introduce a \texttt{guiding network}. 
% %that simultaneously solves unsupervised domain classification and style encoding
% The guiding network consists of a shared trunk with two branches, one of which provides pseudo domain labels, and the other encodes image features.
% % 아래 내용은 Maybe too much for intro?
% % These outputs are later used in the image translation process. For estimating domain labels, we employ a differentiable clustering method that uses a mutual information maximization strategy. This helps the guiding network group similar images together while evenly separating their categories. For learning the image embedding space, we adopt a contrastive loss~\cite{2006contrastive,2019MoCo,2020simclr}. This helps the model to understand the dissimilarity among images and learning better representations. 
% %
% % 이야기 하고 싶은 바: 
% % 구조적으로 도메인 라벨 clustering과 representation learning을 동시에 하게 하다보니, 도메인 라벨 clustering branch도 더 양질의 피드백을 통해 성능이 올라가고, image representation learning branch도 이렇게 잘 뽑힌 (성능이 올라간) domain 정보를 바탕으로 이미지들 간의 차이를 좀 더 잘 이해하게 되므로 더 나은 representation을 배우게 된다. 근데 이게 결국 추후에 생성모델에서 style code로 쓰이게 되기 때문에 좀 더 style을 잘 반영하여 학습하게 하는데 도움이 되고 결과적으로 image translation성능이 좋아진다.
% * By solving two tasks together, the guiding network is encouraged to find a better representation space. This largely improves the  performance of the following image translation model.
% % that is good for both tasks. (shared feature space becomes better?) so that it can provide better feedback to the following generative module.
% % * Since the guiding network has to solve both unsupervised domain classification and representation learning tasks together, it learns better...
% % * Thanks to this interaction between two tasks, our model successfully separates domains and translates images.
% % * By exploiting the synergy of two tasks, the guiding network helps the image translation model to largely improve the generation performance.
% % * We find that the performance of the guiding network largely benefits from solving both unsupervised domain classification and representation learning tasks together. 
% %
% % -- 다음 문단 글감 --
% % Here, we jointly train the guiding network with GAN. Since the guiding network can now exploit gradients from GAN training, it understands the recipes of domain-separating attributes based on GAN's feedback. Thanks to this interaction between the guiding network and GAN, our model successfully separates domains and translates images.
% }

% The style codes are then used to generate a fake sample while the pseudo labels participate in the discriminator's training. 
% Owing to this interactive relationship, the improvement of the guiding network can enhance the overall translation performance. 
% \jj{Because the style codes and the pseudo labels are later used for image translation, the improvement of the guiding network can enhance the overall performance.  we jointly train GAN and the guiding network together although two modules play different roles.} 

% Although GAN and the guiding network play different roles, 

==> Truly unsupervised img2img (arXiv version)/2.related_work.tex <==
\section{Related work}
\label{sec:related_work}
\noindent\textbf{Image-to-image translation.} 
Since the seminal work of Pix2Pix \cite{2017Pix2Pix}, image-to-image translation models have shown impressive results~\cite{2017CycleGAN,2017UNIT,2017DiscoGAN,2017Cycada,2018DeblurGAN,2018StarGAN,2018MUNIT,2019FUNIT,2019DSGAN,2019StarGANv2,wang2020semit}. Exploiting the cycle consistency constraint or shared latent space assumption, these methods were able to train the model with a set-level supervision (domains) solely. However, acquiring domain information can be a huge burden in practical applications where a large amount of data are gathered from several mixed domains, \eg, web images \cite{2019Bilion}. Not only does this complicates the data collection, but it restricts the methods only applicable to the existing dataset and domains. S$^3$GAN~\cite{lucic2019high} and Self-conditioned GAN~\cite{liu2020selfconditioned} integrated a clustering method and GAN for high-quality generation using the fewer number or none of the labeled data, respectively. 
Inspired from few shot learning, Liu \textit{et al.}~\cite{2019FUNIT} proposed FUNIT that works on previously unseen target classes. However, FUNIT still requires the labels for training. Wang \textit{et al.}~\cite{wang2020semit} utilized the noise-tolerant pseudo labeling scheme to reduce the label cost at the training process. Recently, Bahng et al.~\cite{bahng2019exploring} partially addressed this by adopting the ImageNet pre-trained classifier for extracting domain information. Unlike the previous methods, we aim to design an image translation model that can be applied without supervision such as a pre-trained network or supervision on both the train and the test datasets. 
\smallskip\\
\noindent\textbf{Unsupervised representation learning and clustering.} Unsupervised representation learning aims to extract meaningful features for downstream tasks without any human supervision. To this end, many researchers have proposed to utilize the information that can be acquired from the data itself~\cite{2006contrastive,2018RotNet,2018DIM,2019IIC,saunshi2019theoretical,2019MoCo,chen2020simclr,2020SCAN}.
Recently, by incorporating contrastive learning into a dictionary learning framework, MoCo~\cite{2019MoCo,2020mocov2} achieved outstanding performance in various downstream tasks under reasonable mini-batch size. 
On the other hand, IIC~\cite{2019IIC} utilized the mutual information maximization in an unsupervised manner so that the network clusters images while assigning the images evenly. 
Though IIC provided a principled way to perform unsupervised clustering, the method fails to scale up when combined with a difficult downstream task such as image-to-image translation. 
By taking the best of both worlds, we aim to solve unsupervised image-to-image translation.

==> Truly unsupervised img2img (arXiv version)/3.method.tex <==
\section{Truly Unsupervised Image-to-Image Translation (TUNIT)}
\label{sec:method}
\figModel

We address the unsupervised image-to-image translation problem, where we have images $\rchi$ from $K$ domains ($K\geq2$) without domain labels $\y$. Here, $K$ is an unknown property of the dataset. Throughout the paper, we denote $K$ as the actual number of domains in a dataset and $\hat{K}$ as the arbitrarily chosen number of domains to train models. 

\subsection{Overview}
%We design a module, called a guiding network  ($E$ in \Fref{fig:model}). % , which integrates both a domain classifier and a style encoder. 
In our framework, the guiding network ($E$ in \Fref{fig:model}) plays a central role as an unsupervised domain classifier as well as a style encoder. 
% This module extracts the pseudo labels from the source and reference images and the style code from the reference.
It guides the translation by feeding the style code of a reference image to the generator and its pseudo domain labels to the discriminator. Using the feedback from the domain-specific discriminator, the generator synthesizes an image of the target domain (\eg \ breeds) while respecting the style (\eg \ fur patterns) of the reference image and the content (\eg pose) of the source image.

\subsection{Learning to produce domain labels and encode style features}\label{sec:guiding_encoder}
The guiding network $E$ consists of two branches, $\Eclass$ and $\Estyle$, each of which learns to provide domain labels and style codes, respectively. In experiments, we compare our guiding network against straightforward approaches, \ie., K-means on image or feature space.

% \figModel
\smallskip
\noindent\textbf{Unsupervised domain classification.} 
The discriminator requires a target domain label to provide useful gradients to the generator for translating an image into the target domain. %Therefore, we employ a clustering algorithm~\cite{2019IIC} to provide pseudo domain labels for training the discriminator. Because a differentiable clustering method can help the model to understand the similarity within the same domain-- K-means clustering does not affect the representation of the network, 
Therefore, we adopt the differentiable clustering technique~\cite{2019IIC} that maximizes the mutual information (MI) between an image $\x$ and its randomly augmented version $\xp$. 
The optimum of the mutual information $I(\p, \pp)$ is reached when the entropy $H(\p)$ is maximum and the conditional entropy $H(\p|\pp)$ is minimum, where $\p = \Eclass(\x)$ represents the softmax output 
from $\Eclass$, indicating a probability vector of $\x$ over $\hat{K}$ domains. Please refer to Section~\ref{sec:generalizability} for more details about $\hat{K}$.
Maximizing MI encourages $\Eclass$ to assign the same domain label to the pair ($\x$ and $\xp$) while evenly distributing entire samples to all domains. Formally, $\Eclass$ maximizes the mutual information:
\begin{small}
\begin{equation}
\label{eq:iic}
\begin{split}
\mathcal{L}_{MI} &= I(\p, \pp) = I(\P) = \sum_{i=1}^{\hat{K}} \sum_{j=1}^{\hat{K}} \Pij \ln \frac{\Pij}{\P_i \P_j},\\
\textit{s.t.}\ \ \P&=\mathbb{E}_{\xp\sim f(\x) | \x\sim p_{data}(\x)}[\Eclass(\x)\cdot \Eclass(\xp)^T].
\end{split}
\end{equation}
\end{small}
Here, $f$ is a composition of random augmentations such as random cropping and affine transformation. $\P_i=\P(\p=i)$ denotes the $\hat{K}$-dimensional marginal probability vector, and $\Pij=\P(\p=\texttt{argmax}(i), {\pp}=\texttt{argmax}(j))$ denotes the joint probability. To provide a deterministic one-hot label to the discriminator, we use the \texttt{argmax} operation (i.e. $y = \texttt{argmax}(\Eclass(\x))$). Note that the mutual information is one way to implement TUNIT, and any differentiable clustering methods can be adopted such as SCAN~\cite{2020SCAN}.

\smallskip
\noindent\textbf{Style encoding and improved domain classification.} To perform a reference-guided image translation, the generator needs to understand the style features of the given image. In our framework, $\Estyle$ encodes an image into a style code $\s$, which is later used to guide the generator for image translation. Here, to learn the style representation, we use the contrastive loss~\cite{2019MoCo}:
% Though maximizing $\mathcal{L}_{MI}$ provides a way to automatically generate the domain labels for input images, it fails to scale up when the samples become complex and diverse (e.g. AnimalFaces~\cite{2019FUNIT}). We overcome this by adding an auxiliary style encoding branch $\Estyle$ to the guiding network $E$ and imposing the contrastive loss~\cite{2019MoCo}:
\begin{small}
\begin{equation}
\label{eq:contrastive}
\mathcal{L}_{style}^E = -\log\frac{\exp(\s\cdot {\spp}/\tau)}{\sum_{i=0}^N \exp(\s\cdot \sn/\tau)},
\end{equation} 
\end{small}
where $\x$ and $\xp$ denote an image and randomly augmented version of $\x$, respectively, and $\s=\Estyle(\x)$.
This $(N+1)$-way classification enables $E$ to utilize not only the similarity of the positive pair ($\s$, $\spp$) but also the dissimilarity of the negative pairs ($\s$, $\sn$).
We adopt a queue to store the negative codes $\sn$ of the previously sampled images as MoCo~\cite{2019MoCo}. By doing so, we can conduct the contrastive learning efficiently without large batch sizes~\cite{saunshi2019theoretical}.
%where the negative style codes $\sn$ are stored into a queue from the previously sampled images.

Interestingly, we find that $\Estyle$ also helps the unsupervised domain classification task---$(-\mathcal{L}_{MI} + \mathcal{L}_{style}^E)$ significantly improves the quality of the clustering, compared to using only $-\mathcal{L}_{MI}$, which is the original IIC~\cite{2019IIC}. % IIC combined with Eq. \ref{eq:contrastive} ($-\mathcal{L}_{MI} + \mathcal{L}_{style}^E$) significantly improves the quality of the clustering, compared to using the original IIC~\cite{2019IIC} solely. 
Since $\Estyle$ shares the embeddings with $\Eclass$, imposing the contrastive loss on the style codes improves the representation power of the shared embeddings. 
This is especially helpful when samples are complex and diverse, and IIC solely fails to scale up (\eg, AnimalFaces~\cite{2019FUNIT}). 
To evaluate the effect of Eq.\eqref{eq:contrastive}, we measure the accuracy and the ratio of the inter-variance over the intra-variance (IOI) in terms of the cosine similarity of each clustering result. The clustering result can be more discriminative when the intra-variance and the inter-variance become low and high, respectively. Therefore, the higher IOI indicates a more discriminative clustering result. The table below summarizes the accuracies and IOI on AnimalFaces-10 and Food-10. 
\begin{center}
\vspace{-0.5mm}
\tablestyle{10pt}{1.0}
\begin{tabular}{ccc|cc}
& \multicolumn{2}{c}{\textbf{AnimalFaces-10}} & \multicolumn{2}{c}{\textbf{Food-10}} \\
 & IIC & IIC + Eq.\eqref{eq:contrastive} & IIC & IIC + Eq.\eqref{eq:contrastive} \\
\shline
IOI & 2.05 & 3.04 & 1.34 & 2.50 \\
Accuracy & 68.0\% & 85.0\% & 54.2\% & 86.0\% 
\end{tabular}
\vspace{-0.7mm}
\end{center}
For both datasets, IIC with Eq.\eqref{eq:contrastive} shows a significantly higher accuracy and a higher IOI value. Based on this analysis, we choose to use both $-\mathcal{L}_{MI}$ and $ \mathcal{L}_{style}^E$ for training the guiding network. %that our proposed method can improve the quality of the clustering. 
\subsection{Learning to translate images}\label{sec:gan}
We describe how to perform the unsupervised image-to-image translation under the guidance of our guiding network. For successful translation, the model should provide realistic images containing the visual feature of the target domain. To this end, we adopt three losses for training the generator $G$: 1) adversarial loss to produce realistic images, 2) style contrastive loss that encourages the model not to ignore the style codes, 3) image reconstruction loss for preserving the domain-invariant features. We explain each loss and the overall objective for each network.

\smallskip
\noindent\textbf{Adversarial loss.} For adversarial training, we adopt a variant of conditional discriminator, the multi-task discriminator~\cite{mescheder2018r1reg}. It is designed to conduct discrimination for each domain simultaneously. During training, its gradient is calculated only with the loss for estimating the input domain. For the domain label of the input, we utilize the pseudo label from the guiding network. Formally, given the pseudo label $\yt$ for a reference image $\xt$, we train our generator $G$ and multi-task discriminator $D$ via the adversarial loss:
\begin{small}
\begin{equation}
\label{eq:discriminator}
\begin{split}
\mathcal{L}_{adv} &= \mathbb{E}_{\xt\sim p_{data}(\x)}[\log D_{\yt}(\xt)]  \\
& + \mathbb{E}_{\x, \xt \sim p_{data}(\x)}[\log (1 - D_{\yt}(G(\x, \st)))],
\end{split}
\end{equation}
\end{small}
where $D_{\yt}(\cdot)$ denotes the logit from the domain-specific ($\yt$) discriminator, and $\st = \Estyle(\xt)$ denotes a target style code of the reference image $\xt$. The generator $G$ learns to translate $\x$ to the target domain $\yt$ while reflecting the style code $\st$.

\smallskip
\noindent\textbf{Style constrastive loss.} In order to prevent a degenerate case where the generator ignores the given style code $\st$ and synthesize a random image of the domain $\yt$, we impose a style contrastive loss:
\begin{small}
\begin{equation}
\label{eq:stycontrastive}
\mathcal{L}_{style}^G = \mathbb{E}_{\x, \xt \sim p_{data}(\x)}\left[-\log\frac{\exp(\stt \cdot \st)}{\sum_{i=0}^N \exp(\stt \cdot \sn/\tau)}\right].
\end{equation}
\end{small}
Here, $\stt = \Estyle(G(\x, \st))$ denotes the style code of the translated image $G(\x, \st)$ and $\sn$ denotes the negative style codes, which are from the same queue used in Eq.~\eqref{eq:contrastive}. Besides, the same training scheme of MoCo~\cite{2019MoCo} is applied for the generator training as Eq.~\eqref{eq:contrastive}. This loss guides the generated image $G(\x, \st)$ to have a style similar to the reference image $\xt$ and dissimilar to negative (other) samples. By doing so, we avoid the degenerated solution where the encoder maps all the images to the same style code of the reconstruction loss~\cite{2019StarGANv2} based on L1 or L2 norm. Eqs.~\eqref{eq:contrastive} and \eqref{eq:stycontrastive} are based on contrastive loss, but they are used for different purposes. Please refer to Appendix 12. for more discussion.

\smallskip
\noindent\textbf{Image reconstruction loss.} We impose that the generator $G$ can reconstruct the source image $\x$ when given with its original style $\s = \Estyle(\x)$, namely an image reconstruction loss:
\begin{small}
\begin{equation}
\label{eq:reconstruction}
\mathcal{L}_{rec} = \mathbb{E}_{\x\sim p_{data}(\x)}[\lVert \x - G(\x, \s) \rVert_1].
\end{equation}
\end{small}
This objective not only ensures the generator $G$ to preserve domain-invariant characteristics (e.g., pose) of its source image $\x$, but also helps to learn the style representation of the guiding network $E$ by extracting the original style $\s$ of the source image $\x$.

\smallskip
\noindent\textbf{Overall objective.} Finally, we train the three networks jointly as follows:
\begin{small}
\begin{equation}
\label{eq:totobjectives}
\begin{split}
\mathcal{L}_D &= -\mathcal{L}_{adv}, \\
\mathcal{L}_G &= \mathcal{L}_{adv} + \lambda_{style}^G\mathcal{L}_{style}^G + \lambda_{rec}\mathcal{L}_{rec}, \\
\mathcal{L}_E &= \mathcal{L}_G-\lambda_{MI}\mathcal{L}_{MI} + \lambda_{style}^E\mathcal{L}_{style}^E
\end{split}
\end{equation}
\end{small}
where $\lambda$'s are hyperparameters. Note that our guiding network $E$ receives feedback from $L_{G}$, which is essential for our method. We discuss the effect of feedback to $E$ on performance in Section~\ref{sec:comparison}.

==> Truly unsupervised img2img (arXiv version)/4.experiments.tex <==
\section{Experiments}
\label{sec:experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                Experiment intro                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tabmain
\figmaincomparison
\tabKcomparisonn
\figFFHQfew
\tabsemi
% We first evaluate TUNIT on labeled datasets by treating them as unlabeled because the desired behaviours of the translation models in labeled datasets are well defined~(\Sref{sec:comparison}). Here, we provide an ablation study to analyze the effect of each component and compare the models both quantitatively and qualitatively. 
We first investigate the effect of each component of TUNIT~(\Sref{sec:comparison}). We quantitatively and qualitatively compare the performance on labeled datasets. We show that TUNIT is robust against the choice of hyperparameters (e.g. the preset number of clusters, $\tilde{K}$) and extends well to the semi-supervised scenario~(\Sref{sec:generalizability}). Lastly, we move on to unlabeled datasets to validate our model in the unsupervised scenario in the wild~(\Sref{sec:unsupervised}). 

% In all experiments, we use FUNIT~\cite{2019FUNIT} as our baseline and we also compare TUNIT with SEMIT~\cite{wang2020semit} for the semi-supervised scenario.

\medskip
\noindent\textbf{Datasets.} 
For the labeled datasets, we select ten classes among 149 classes of AnimalFaces and 101 classes of Food-101, which we call AnimalFaces-10 and Food-10, respectively. Here, the labels are used only for the evaluation purpose except for the semi-supervised setting. For the unlabeled datasets, we use AFHQ, FFHQ, and LSUN Car~\cite{2019StarGANv2,2019StyleGAN,2015LSUN}, which do not have any or are missing with fine-grained labels. Specifically, AFHQ roughly has three groups (\ie, dog, cat and wild), but each group contains diverse species and these species labels are not provided. FFHQ and LSUN Car contain various human faces and cars without any labels, respectively.

\medskip
\noindent\textbf{Evaluation metrics.} We report two scores to assess the generated images. First, to provide a general sense of image quality, we use the mean of class-wise Fr\'enchet Inception Distance (mFID)~\cite{2017FID}. It can avoid the degenerate case of the original FID, which assigns a good score when the model conveying the source image as is. Additionally, to provide a finer assessment of the generated images, we report Density and Coverage (D\&C)~\cite{2020DnC}. D\&C separately evaluates the fidelity and the diversity of the model outputs, which is also known to be robust against outliers and model hyperparameters (e.g. the number of samples used for evaluation). A lower mFID score means better image quality, and D\&C scores that are bigger or closer to 1.0 indicate better fidelity and diversity, respectively. Please refer to Appendix 3. for the detailed information.
% to assess the model outputs in more detail, which separately analyze the fidelity and diversity of the images. 
% to avoid the degenerate identity output case getting a good score---the model conveys the source image as is, which cannot be discriminated by using the original FID
% Using D\&C, we can separately assess the fidelity and diversity of the model outputs, which again complements the blind sight of the mFID score.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                Experiment Comparison                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparative Evaluation on Labeled Datasets}
% \figKcomparison
\label{sec:comparison}
\Tref{tab:main} summarizes the effect of each component of TUNIT and rigorous comparisons with the state-of-the-art supervised method, FUNIT. First, we report the set-level supervised performance of FUNIT and its variant (\Tref{tab:main}). Here, \texttt{A} is the original FUNIT and \texttt{B} denotes the modified FUNIT using our architecture (\eg we do not use PatchGAN discriminator), which brings a large improvement over every score on both datasets. 
One simple way to extend \texttt{B} to the unsupervised scenario is to add an off-the-shelf clustering method and use its estimated labels instead of the ground truth. We employ K-means clustering on the image space for \texttt{C}, and the pretrained feature space for \texttt{D}. Here, we use ResNet-50~\cite{2016resnet} features trained with MoCo v2~\cite{2020mocov2} on ImageNet. Not surprisingly, because the estimated labels are inaccurate, the overall performance significantly drops. 
Although using the pretrained features helps a little, not only is it far from the set-level supervised performance but it requires three steps to train the entire model, which complicates the application. This can be partially addressed by employing the differentiable clustering method~\cite{2019IIC}, which trains VGG-11BN~\cite{2014VGG} with mutual information maximization from scratch that makes \texttt{E}. This reduces the number of training steps from three to two and provides better label estimation, which enables the model to approach the performance of original FUNIT \texttt{A}. However, as seen in the coverage score, the sample diversity is unsatisfactory. 

Finally, we build TUNIT by introducing the guiding network and the new objective functions described in \Sref{sec:method}. The changes significantly improve the accuracy on both datasets, particularly achieving similar mFID of the improved set-level supervised model \texttt{B}. Our final model, \texttt{G} matches or outperforms mFID and D\&C of \texttt{B}. This is impressive because \texttt{B} utilizes oracles for training while \texttt{G} has no labels. Notably, TUNIT can improve the coverage by 0.073 (7\%p) on AnimalFaces-10 than \texttt{B}. 
We conjecture that TUNIT benefits from the guiding network, which jointly learns the style encoding and clustering with the shared encoder. Because their clustering modules are as powerful as TUNIT, the performance drawback of \texttt{C}, \texttt{D} and \texttt{E} supports that the feedback from style encoding is a key success factor of TUNIT. By comparing \texttt{F} and \texttt{G}, we confirm that they are comparable in terms of clustering and \texttt{G} is more stable in terms of inter-dataset performance. Therefore, we adopt the joint training of style encoder and clustering as our final model (\texttt{G}). In addition, we investigate the effect of joint training between GAN and the guiding network by removing the adversarial loss for training the guiding network. It directly degrades the performance; mFID changes from 47.7 to 63.0 on AnimalFaces-10. It indicates that our training scheme takes an important portion of performance gains. Qualitative results also show the superiority of TUNIT over competitors~(\Fref{fig:main_comparison}).
% Finally, we build TUNIT by introducing the guiding network having two branches and the new objective functions described in \Sref{sec:method}. To investigate the effect of joint training in TUNIT, we constitute the model \texttt{F} for sequential training of style encoder and clustering network, and the model \texttt{G} for joint training of them. The results demonstrate that the changes in model architecture and objectives significantly improve the accuracy on both datasets, particularly achieving nearly the same mFID of the supervised model \texttt{B}. Our final model \texttt{G} matches or outperforms mFID and D\&C of \texttt{B}. This is impressive because \texttt{B} utilizes oracles for training while \texttt{G} has no labels both for training and testing. Particularly, TUNIT can cover 7\%p wider support of the data on AnimalFaces-10 than \texttt{B}. We conjecture that the remarkable performance of TUNIT benefits from the style codes representing meaningful domain features learned by clustering, which eventually leads to a better translation model. Comparing \texttt{F} and \texttt{G}, we confirm that the joint training scheme improves overall performances. To observe the effect of the interactive training between GAN and guiding network, we degenerate TUNIT by removing the gradient of adversarial loss for training the guiding network. This change directly degrades the translation performance; mFID changes from 47.7 to 63.0 on AnimalFaces-10. This large gap indicates that our interactive training scheme takes an important portion of performance gains. Qualitative results also shows superiority of TUNIT over competitors~\Fref{fig:main_comparison}.
% For the qualitative evaluation, please refer to \Fref{fig:main_comparison}.
% Qualitative
% We also conduct the qualitative evaluation of \texttt{A}-\texttt{G} on the labeled datasets as shown in \Fref{fig:main_comparison}. Here, \texttt{B} reflects the style feature (\eg species or type of food) of the reference images while \texttt{A} does not. 
% The model \texttt{C} performs much worse than \texttt{A} and \texttt{B} in that it overly adopts the source image, not adequately merging styles and contents from both sides. The model \texttt{D} generates more plausible images than \texttt{C} but fails to reflect the characteristics of the reference images. For example, \texttt{D} on fifth row does not look like \emph{several pieces of dumpling} due to its shape and dish color, meaning that the reference styles are not properly reflected. % contains separated individual chunks but the result looks a single chunk and the output of the last row does not reflect even the color of the reference. 
% Similarly, \texttt{E} also fails to generate the dumpling in the fifth row. % also works reasonably for many cases but still, it does not translate the food on fifth row at all.
% TUNIT with sequential training \texttt{F} reflects the visual features of each reference on both datasets. However, in terms of visual fidelity, we observe that \texttt{G} consistently  outperforms \texttt{F}. Akin to the quantitative results, TUNIT achieves equivalent or even better visual quality than the supervised model \texttt{A} and \texttt{B}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                Experiment Generalizability                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\figUnlabeled
\figtsnecompare
\subsection{Analysis on Generalizability}
\label{sec:generalizability}
\noindent\textbf{Robustness to various $\hat{K}$'s.} When TUNIT conducts clustering for estimating domain labels, the number of clusters $\hat{K}$ can affect the performances. Here, we study the effects on different $\hat{K}$ on the labeled datasets and report them in \Tref{tab:k_comparison}. For the qualitative comparison, please refer to Appendix 1. As expected, the model performs best in terms of mFID when $\hat{K}$ equals to the ground truth $K$ (\ie $\hat{K}$=10). 
%Additionally, TUNIT performs reasonably well for sufficiently large \textcolor{red}{$\hat{K}$} ($\geq 7$) on both datasets. Even though we set $\hat{K}$ to 100 times larger than the actual number of the domains, TUNIT still works well. From this study, we conclude that TUNIT is relatively robust against \textcolor{red}{$\hat{K}$} as long as it is sufficiently large.

One thing to note here is that TUNIT performs reasonably well for a sufficiently large $\hat{K}$ ($\geq 7$). More interestingly, even with 100 times larger $\hat{K}$ than the actual number of the domains, TUNIT still works well on both datasets. This trend is also seen in the t-SNE visualization(~\Tref{tab:k_comparison}). From this study, we conclude that TUNIT is relatively robust against $\hat{K}$ as long as it is sufficiently large. Thus, in practice, we suggest to use a sufficiently large $\hat{K}$ or to study different $\hat{K}$'s in log scale for finding the optimal model. 
% \tabsemicls

\medskip
\noindent\textbf{With Few labels.} We also investigate whether or not TUNIT is effective for a more practical scenario, semi-supervised image translation. To utilize the labels, AnimalFaces and Food datasets are chosen for this experiment. Specifically, AnimalFaces-10 and Food-10 are used for evaluating the models on the small datasets while AnimalFaces-149 and Food-101 are used for assessing the models on the large datasets. We partition the dataset $\mathcal{D}$ into the labeled set $\mathcal{D}_{sup}$ and the unlabeled set $\mathcal{D}_{un}$ with varying ratio $\gamma=|\mathcal{D}_{sup}|/|\mathcal{D}|$. For the semi-supervising setting, we train $\Eclass$ of TUNIT by an additional cross-entropy loss between the ground truth domain labels and the predicted domain labels on $\mathcal{D}_{sup}$. Besides, the true domain labels for $\mathcal{D}_{sup}$ are utilized for training the domain-specific discriminator. 
As a counterpart in this scenario, FUNIT~\cite{2019FUNIT} and SEMIT~\cite{wang2020semit} are selected because both models can be applied to the semi-supervised image translation (SEMIT achieves the current state-of-the-art performance in the semi-supervised setting). We train the two competitors and TUNIT by changing $\gamma$ from 0.01 to 0.8 and report the results in \Tref{tab:semi_wo_cls}. For the small datasets, the performance of FUNIT significantly degrades as $\gamma$ decreases. Meanwhile, TUNIT and SEMIT produce relatively similar mFID scores despite $\gamma$ decreases. Even when SEMIT maintains mFID, TUNIT significantly outperforms SEMIT by 20\% of mFID on small datasets. For the large datasets, TUNIT either outperforms or is comparable to the competitors. Especially, on AnimalFaces-149, TUNIT clearly outperforms both competitors. By the experiments on the semi-supervised setting, we conclude that TUNIT can be easily adapted to the semi-supervised image translation with the simple modification (\ie adding the supervised training on the labeled samples), and serve as a strong baseline model. As a result, TUNIT for the semi-supervised setting achieves impressive performance, which is comparable to the state-of-the-art semi-supervised translation method. We provide the qualitative comparison in the appendix.

\subsection{Validation on Unlabeled Dataset}
\label{sec:unsupervised}

Finally, we evaluate TUNIT on the unlabeled datasets (AFHQ, FFHQ and LSUN-Car), having no clear separations of the domains. For AFHQ, we train three individual models for \emph{dog}, \emph{cat} and \emph{wild}. For all experiments, we use FUNIT as a baseline, where all the labels for training are regarded the same as one. We set the number of clusters $\hat{K}$=10 for all the TUNIT models. 
% Please refer to \Sref{sec:generalizability} for the effect of different $\hat{K}$.
% More discussions on $\hat{K}$ will be in \Sref{sec:generalizability}. 
% Because of the page limit, we include AFHQ-\emph{wild} and LSUN-Car in main text. For more results, please refer to \Aref{sec:app_tsne}, \ref{sec:app_additional_examples}. 

% The upper side of figure~\ref{fig:unlabeled_reference_guided} demonstrates the results. We observe that the results of TUNIT adequately reflect the style feature of the references such as the textures of cars and the species of the wilds. However, FUNIT performs much worse than TUNIT in this truly unsupervised scenario. For example, FUNIT outputs the inputs as is (wilds) or insufficiently reflects the species (third row of AFHQ Wild).  
Figure~\ref{fig:unlabeled_reference_guided} demonstrates the results. We observe that the results of TUNIT adequately reflect the style feature of the references such as the textures of cats or cars and the species of the wilds. Although FFHQ has no clear domain distinctions, TUNIT captures the existence of glasses or smile as domains, and then add or remove glasses or smile. However, FUNIT performs much worse than TUNIT in this truly unsupervised scenario. For example, FUNIT outputs the inputs as is (cats and wilds) or insufficiently reflects the species (third row of AFHQ Wild). For FFHQ, despite that FUNIT makes some changes, the changes are not interpreted as meaningful domain translations. For LSUN Car, FUNIT fails to keep the fidelity. 

We also visualize the style space of both models to qualitatively assess the quality of the representation. \Fref{fig:tsne_compare} shows the t-SNE maps trained on AFHQ Wild and the examples of each cluster; the sample color corresponds to the box color of representative images. Surprisingly, TUNIT organizes the samples according to the species where it roughly separates the images into six species. Although we set $\hat{K}$ to be overly large, the model represents one species into two domains where those two domains position much closely (\eg tiger). From these results, we confirm that the highly disentangled, meaningful style features can be an important factor in the success of our model. 
On the other hand, the style features of FUNIT hardly learn meaningful domains so that the model cannot conduct the translation properly as shown in \Fref{fig:unlabeled_reference_guided}. 
Because of the page limit, we include more results including qualitative comparison and the t-SNE visualization in Appendix 8,9,10 and 11.

% \figUnlabeled
% \figtsnecompare
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                Experiment Comparison                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
    In this section, we present three experiments: analyzing the effect of the proposed objective functions and training strategy~(\Sref{sec:analysis}), an unsupervised image-to-image translation on three unlabeled datasets~(\Sref{sec:unsupervised}), and comparison to the state-of-the-art (SOTA) techniques under a semi-supervised setting~(\Sref{sec:semisupervised}). For quantitative evaluation, we use Fr\'enchet Inception Distance (FID)~\cite{2017FID}. Because FID cannot penalize the case when the model conveys the source image as is for the output image, we calculate mean of class-wise FID. For the details, please see the supplementary material.
    
    \smallskip
    
    \noindent\textbf{Baselines.} We use FUNIT~\cite{2019FUNIT} and MSGAN~\cite{2019MSGAN}, which are the SOTA multi-domain and cross-domain image-to-image translation models, respectively. For the stable training of FUNIT, we slightly change the architecture of its discriminator from PatchGAN to non-PatchGAN setting. 
    Under the semi-supervised scenario, we compare our method with both baselines in two training schemes. One is a na\"ive scheme that utilizes only the subset of the labeled dataset for entire training. And the other is to train a simple domain classifier using the labeled data and utilize its domain output of the unlabeled data so that GANs can be trained with the whole images (\Sref{sec:semisupervised}).
    
    \smallskip
    
    \noindent\textbf{Datasets.} For unsupervised translation, we evaluate our method on AFHQ, FFHQ, and LSUN Cars datasets~\cite{2019StarGANv2,2019StyleGAN,2015LSUN}. Note that these datasets do not have fine-grained set-level labels.
    AFHQ consists of three roughly labeled classes (i.e., dog, cat and wild), where each class contains diverse species. FFHQ and LSUN Car contain various kinds of human faces and cars, respectively. For comparing with previous methods, we conduct the semi-supervised scenario by varying the supervision levels. Here, we use AnimalFaces~\cite{2019FUNIT} (multi-domain) and Summer2winter (cross-domain).
    Among total 149 animal classes from AnimalFaces, ten classes are chosen arbitrarily for training and testing. We call the selected dataset as AnimalFaces-10.
    
    % remove
    % \graphTwoStepVsJoint
    % \graphLossAblation
    
    \smallskip
    
    \subsection{Effect of our training strategy}
    \label{sec:analysis}
    In this section, we investigate the effect of our training strategy, which simultaneously performs representation learning as well as training the translation networks. Though one can easily think of separately training the guiding network and GANs, we show that this significantly degrades the overall performance. For this analysis, we choose AnimalFaces-10 and compare two training strategies with the proposed model; 1) joint training and 2) separate training. More specifically, the former is to train all the networks in an end-to-end manner as described in~\Sref{sec:method}, and the latter is to first train the guiding network with $\mathcal{L}_{MI}$ and $\mathcal{L}_{style}^C$ for 100k iterations and then train the generator and the discriminator using the outputs of the frozen guiding network as their inputs. Note that for the separate training, the guiding network does not receive feedback from the translation loss $\mathcal{L}_G$ in Eq.\eqref{eq:totobjectives}.
    
        
    To analyze the effects of different training strategies, we plot the class-wise FID over training iteration and provide t-SNE visualization in Fig.~\ref{fig:two_step_vs_joint}. From the FID comparison, the separate training strategy records much higher average FID score with higher standard deviation than the joint training strategy. This clearly shows that the joint training is more effective in terms of the image quality and the stable performance. To understand the performance gain by the joint training strategy, we visualize the style space of the guiding network via t-SNE. Here, the accuracy of the guiding network for each strategy is 83.6\% and 70.4\%, respectively. When the model is trained in the end-to-end manner, the clusters become more compact and clearly separated. Meanwhile, the separate training strategy leads the feature space to be entangled with significant overlaps. From this observation, we conclude that our joint training strategy induces more compact and disentangled clusters, thereby the generator can benefit from the style codes representing meaningful domain features, which eventually leads to the better translation model.
    
    Under the joint training strategy, we study the effect of each component ($\mathcal{L}_{adv}$, $\mathcal{L}_{rec}$, $\mathcal{L}_{style}^G$) in $\mathcal{L}_G$ for the guiding network on the translation performance. We train the model while excluding one of the losses one at a time when training the guiding network. 
    Fig.~\ref{fig:loss_ablation} shows the FID curves over training iterations for each setting. Removing $\mathcal{L}_{rec}$ or $\mathcal{L}_{style}^G$ does not show a meaningful impact on the translation performance. However, removing $\mathcal{L}_{adv}$ drops the translation performance significantly. We conjecture that it is because the adversarial loss cares not only how realistic the output images are but also their domains. From the experiment, we verify that the adversarial loss imposed to the guiding network enhances the overall translation performance of our model.
    
    From the study on the training strategy, we confirm that the interaction between the guiding network and GANs indeed enhances the translation performance. Therefore, in the following experiments, we adopt the joint training scheme and update the guiding network with full $\mathcal{L}_G$.
    
    % remove or app or other dataset
    % \figTSNE
    \subsection{Image-to-image translation without any labels}
    \label{sec:unsupervised}
    
    To verify that the proposed method is able to handle unsupervised image-to-image translation, we evaluate our model on AFHQ, FFHQ and LSUN Car datasets. Only for AFHQ, we utilize the rough labels; dog, cat, and wild through training three sets individually, which means that we train one model per each domain of AFHQ. Because none of previous techniques consider a truly unsupervised image-to-image translation problem, we solely evaluate the proposed method on these datasets. For all datasets, we do not know the exact number of classes. Therefore, we arbitrarily set the number of domains ($K$) to 10 assuming these are sufficiently large to cover the hidden classes. Interestingly, we find that our method shows consistent performance across different $K$'s.  
    % remove or app
    % \figAfhq
    % \figOthers
    
    Because the datasets do not contain fine labels, we cannot conduct quantitative evaluation for this experiment. Instead, we visualize the style space from the guiding network to qualitatively assess the quality of representation learning. Fig.~\ref{fig:tsne_afhq} shows the t-SNE result of the guiding network trained on AFHQ \textit{wild} class and the example images from each domain. Surprisingly, the guiding network organizes the samples according to the species where it roughly separates the AFHQ wild images into seven species. Although we set the number of domains to be overly large, the network represents one species into two domains where those two domains position much closely. Thanks to this highly disentangled style space, our model can successfully handle the unsupervised image-to-image translation problem. The qualitative image translation results are demonstrated in Fig.~\ref{fig:ours_qualitative_afhq}. Each image is synthesized with the source image and the average style code of all test images in each domain. Four representative images of each domain are shown above. We consistently observe that each output successfully reflects the visual feature of each domain (\textit{i.e.} the fur pattern and the color) and the visual feature of its species. The results from FFHQ and LSUN Car are shown in Fig.~\ref{fig:ours_qualitative_others}. Though it is not clear how to define the `domains' in FFHQ, the network successfully separates the images into the visually distinctive categories such as glasses, hair color, and bang. For LSUN Car, the color of output images seamlessly follows the color of the reference images while preserving the type of the source images. Please refer to the supplementary material for t-SNE visualizations, reference-guided translation results for all the datasets, and images representing each domain for FFHQ and LSUN Car. 
    
    % \figAnimalFacesCluster
    \subsection{Image-to-image translation with fewer labels}
    \label{sec:semisupervised}
    In this section, we compare our model to the state-of-the-art translation models trained in two schemes under the semi-supervised learning setting. We partition the dataset $\mathcal{D}$ into the labeled set $\mathcal{D}_{sup}$ and the unlabeled set $\mathcal{D}_{un}$ with varying ratio $\gamma=|\mathcal{D}_{sup}|/|\mathcal{D}|$. The first scheme is to train the models na\"ively using only $\mathcal{D}_{sup}$. The second scheme is proposed to address the unfairness of the number of usable samples for training translation models. Here, an auxiliary classifier is trained on $\mathcal{D}_{sup}$ and is employed to produce pseudo-labels for $\mathcal{D}_{un}$. Using these labels, the translation model can be trained on the entire $\mathcal{D}$. Unlike these competitors, our model always utilize the entire dataset $\mathcal{D}$ by estimating pseudo labels via the guiding network. In the semi-supervised setting, the proposed model exploits an additional cross-entropy loss between the ground truth and the probability vector on $\mathcal{D}_{sup}$ for training $\Eclass$. By employing powerful few-shot or semi-supervised learning algorithms to improve the classifier, one might be able to improve the image-to-image translation model with fewer labels~\cite{2020Fixmatch,2019FewShot}. Though this is an interesting direction, we leave it as a future research topic.
    
    \smallskip
    % \figAnimalFaces
    % remove
    % \graphPartial
    
    % \figSummerWinter
    \noindent\textbf{Na\"ive scheme.} Fig.~\ref{fig:graph_partial} (a) and (b) demonstrate the quantitative results using the class-wise FID on Summer2winter and AnimalFaces-10, respectively. As the ratio ($\gamma$) decreases, the performance of baseline models significantly degrades while the proposed model maintains FID around 60 and 45 regardless of $\gamma$. More importantly, the proposed model trained with only 5\% outperforms MSGAN with all the labels (FID scores of 59.5 vs 77.2 on Summer2winter) and is comparable to FUNIT (FID scores of 42.7 vs 46.2 on AnimalFaces-10) with the entire dataset. Fig.~\ref{fig:compare_animal_faces} shows the qualitative comparisons between our results and the baselines trained with na\"ive scheme. We generate the translated images from the same reference but with the different $\gamma$ and from the different references with the different $\gamma$. The results from FUNIT and MSGAN have poor quality for 5\% labels and contain artifacts for even 30\% labels.
    
    \noindent\textbf{Alternative scheme.} The baseline trained with na\"ive scheme does not fully utilize the training samples as it simply disregards $\mathcal{D}_{un}$.
    To better exploit the entire training samples, we train an auxiliary classifier with $\mathcal{D}_{sup}$ from scratch to produce pseudo labels for $\mathcal{D}_{un}$. We vary the ratio of labeled data ($\gamma$) from 0\% to 10\% (0\% is only for our method). We use VGG11-BN network~\cite{2014VGG} for both datasets. We note that the architecture of guiding network is also VGG11-BN network, therefore this is fair comparison. Fig.~\ref{fig:graph_cls_summer2winter} plots FID versus $\gamma$. Similar to the na\"ive scheme, the proposed model significantly outperforms MSGAN across all $\gamma$'s. Interestingly, the performance of MSGAN using the alternative training is no longer sensitive to the changes in $\gamma$. Fig.~\ref{fig:graph_cls_animal_faces} shows both the classification accuracy and FID scores on AnimalFaces-10. The accuracy of auxiliary classifier improves as the number of training samples (with labels) increases. The translation quality naturally improves upon the higher classification accuracy. Although the classification accuracy of the ratio 8\% case for FUNIT and 1\% case for our model are similar (around 86\%), the translation performance shows a noticeable gap (59.6 for FUNIT and 47.9 for our model). It implies that the accuracy is not the only factor for governing the translation performance. 
    Based on our extensive comparisons and evaluations, we show that the proposed model is effective for the semi-supervised scenario and outperforms the baselines with the significant improvements.
\fi

==> Truly unsupervised img2img (arXiv version)/5.conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We argue that an unsupervised image translation should denote a task that does not utilize any kinds of supervision, neither image-level (\ie paired) nor set-level (\ie unpaired). In this regime, most of the previous studies fall into the set-level supervised framework, using the domain information at a minimum. 
In this paper, we proposed TUNIT, a truly unsupervised image translation method. 
By exploiting synergies between clustering and representation learning, TUNIT finds pseudo labels and style codes so that it can translate images without using any external information. 
The experimental results show that TUNIT can successfully perform an unsupervised image translation while being robust against hyperparameter changes (\eg, the preset number of clusters, $\hat{K}$). Our model is easily extended to the semi-supervised setting, providing comparable results to the state-of-the-art semi-supervised method. These highlight TUNIT has great potential in practical applications.

% To this end, we designed the guiding network that performs unsupervised clustering and representation learning for providing pseudo labels and the style codes for image translation. 
% To this end, we designed the guiding network that performs unsupervised clustering and representation learning together so as to provide pseudo labels and style codes for image translation. By exploiting synergies between two tasks, our guiding network enables the generator to conduct the unsupervised image translation. 
% 원본
% We argue that the unsupervised image translation should not utilize any supervision, such as image-level (\ie paired) or set-level (\ie unpaired) supervision. Under this rigorous regime, many previous studies fall into the set-level supervised framework that uses the domain information at a minimum. In this paper, for the first time, we proposed an effective model to handle the truly unsupervised image translation. To this end, we suggested the guiding network that performs unsupervised clustering and representation learning for providing pseudo labels and the style codes for the image translation. The experimental results showed that guiding network indeed exploits the synergy between two tasks, and the proposed model successfully conducts the unsupervised translation. We showed that our model is relatively robust against $\hat{K}$. In addition, TUNIT can easily extend to the semi-supervised setting and be comparable to the state-of-the-art semi-supervised method. These  highlight the great potential of TUNIT on practical applications.  

==> Truly unsupervised img2img (arXiv version)/abstract.tex <==
% \twocolumn[{
% \renewcommand\twocolumn[1][]{#1}
% \maketitle
% \vspace{-0.7 cm}
% \begin{center}
%     \centering 
%     \vspace{-0.0 cm}
%     \includegraphics[width=1\textwidth]{teaser_3row.pdf}
%     \captionof{figure}{Our model is able to conduct image-to-image translation without any supervision. The output images are generated with the source image and the average style code of each estimated domain. The breed of the output cat changes according to the domain while preserving the pose of the source image.} 
%     \label{fig:teaser}
% \end{center}
% }]
\begin{abstract}
\vspace{-0.3cm}
Every recent image-to-image translation model inherently requires either image-level (\ie input-output pairs) or set-level (\ie domain labels) supervision. However, even set-level supervision can be a severe bottleneck for data collection in practice. In this paper, we tackle image-to-image translation in a fully unsupervised setting, \ie, neither paired images nor domain labels. To this end, we propose a truly unsupervised image-to-image translation model (TUNIT) that simultaneously learns to separate image domains and translates input images into the estimated domains. 
Experimental results show that our model achieves comparable or even better performance than the set-level supervised model trained with full labels, generalizes well on various datasets, and is robust against the choice of hyperparameters (\eg the preset number of pseudo domains). Furthermore, TUNIT can be easily extended to semi-supervised learning with a few labeled data. The source code is available at \url{https://github.com/clovaai/tunit}.
\end{abstract}
\vspace{-0.0 cm}

==> Truly unsupervised img2img (arXiv version)/figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                    Teaser                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figteaser}{
\vspace{-0 cm}
\begin{center}
    \centering 
    \vspace{-1mm}
    \includegraphics[width=1\textwidth]{figures/section1/teaser_3row.pdf}
    % \includegraphics[width=0.95\textwidth]{figures/section1/afhq_cat_cluster_3row.pdf}
    \captionof{figure}{\small{Our model is able to conduct image-to-image translation without any supervision. The output images are generated with the source image and the the average style code of each estimated domain. The breed of the output cat changes according to the domain while preserving the pose of the source image.}} 
    \label{fig:teaser}
\end{center}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                 Introduction                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figIntro}{
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{intro_figure_notext.pdf}
\vspace{-0.1cm}
\makebox[0.2\linewidth][c]{\footnotesize{(a) Image-level}}\hfill
\makebox[0.45\linewidth][c]{\footnotesize{(b) Set-level}}\hfill
\makebox[0.35\linewidth][c]{\footnotesize{(c) Unsupervised}}\hfill \\
\caption{\small{\textbf{Levels of supervision.} To perform image-to-image translation, existing methods need either \textbf{(a)} a dataset with input-output pairs or, \textbf{(b)} a dataset with domain information. Our method is capable of learning mappings among multiple domains using \textbf{(c)} a dataset without any supervision.}} 
%(\textcolor{red}{Here in (c), what is the key message to deliver? do we want to say that multiple possible categories can be drawn from a unsupervised setting? or the definition of domains is ambiguous or noisy? It is not clear a selling point.   }).



%\textbf{(a)} Dataset with input-output pairs.
%\textbf{(b)} Dataset with domain information.
%\textbf{(c)} Dataset with neither paired data nor domain labels.
% \textbf{(a)} Image-level supervised methods require input-output pairs.
% \textbf{(b)} Set-level supervised methods do not require paired data but domain labels.
% \textbf{(c)} Unsupervised methods require neither paired data nor domain labels.


\label{fig:introduction}
\vspace{-0.3cm}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                   Section 3                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figModel}{
\newcommand{\h}{0.9\columnwidth}
\begin{figure}[t!]
\centering
\includegraphics[width=\h]{training_overview_column_2.jpg}\\
\caption{\small{\textbf{Overview of our proposed method.} The figure illustrates how our model changes the breed of a cat. \textbf{(a)} Our guiding network $E$ estimates the domain and use it to train the multi-task discriminator $D$. \textbf{(b)} Both the style code and the estimated domain of a reference image is used for training the generator $G$.}
}
\label{fig:model}
\vspace{-0.5 cm}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Section 4                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figmaincomparison}{
\renewcommand{\h}{14.0mm}
\newcommand{\hout}{13.56mm}
\begin{figure*}[t]
\centering
\footnotesize{
\makebox[\h][c]{Source}\hspace{-0.3mm}
\makebox[\h][c]{Reference}\hspace{0.9mm}
\makebox[\hout][c]{\arch{\normalsize a}}\hspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize b}}\hspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize c}}\vspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize d}}\hspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize e}}\hspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize f}}\vspace{0.0mm}
\makebox[\hout][c]{\arch{\normalsize g}}\hspace{0.0mm}
\vspace{0.3mm}
}\\\
\includegraphics[width=130mm]{model_comparison.jpg}
\vspace{-2mm}
\caption{\small{Qualitative comparison of translation results using each configuration in \Tref{tab:main}. 
%TUNIT (\arch{f}) - (\arch{g}) successfully reflects the visual appearance of each reference in all cases. We also conduct the qualitative evaluation of \texttt{A}-\texttt{G} on the labeled datasets as shown in \Fref{fig:main_comparison}. 
Here, \texttt{B} reflects the style feature (\eg species or type of food) of the reference images while \texttt{A} does not. 
The model \texttt{C} performs much worse than \texttt{A} and \texttt{B} in that it overly adopts the source image, not adequately merging styles and contents from both sides. The model \texttt{D} generates more plausible images than \texttt{C} but fails to reflect the characteristics of the reference images. For example, \texttt{D} on fifth row does not look like \emph{several pieces of dumpling} due to its shape and dish color, meaning that the reference styles are not properly reflected. 
Similarly, \texttt{E} also fails to generate the dumpling in the fifth row. 
TUNIT with sequential training \texttt{F} reflects the visual features of each reference on both datasets. However, in terms of visual fidelity, we observe that \texttt{G} consistently  outperforms \texttt{F}. Akin to the quantitative results, TUNIT achieves equivalent or even better visual quality than the set-level supervised model \texttt{A} and \texttt{B}.}
}
\vspace{-4mm}
\label{fig:main_comparison}
\end{figure*}
}

% appendix
\newcommand{\figKcomparison}{
% 15 / 14.5
\renewcommand{\h}{14.0mm}
\renewcommand{\hout}{13.56mm}
\begin{figure*}[t!]
\centering
\vspace{-2mm}
\footnotesize{
\makebox[\h][c]{Source}\hspace{0.0mm}
\makebox[\h][c]{Reference}\hspace{0.7mm}
\makebox[\hout][c]{$\hat{K}$=1}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=4}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=7}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=10}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=13}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=16}\hspace{0.0mm}
\makebox[\hout][c]{$\hat{K}$=20}\hspace{0.0mm}
}\\\
% 139
\includegraphics[width=130mm]{k_comparison.jpg}
\vspace{-2mm}
\caption{\small{Qualitative comparison on the number of pseudo domains $\hat{K}$. The performance varies along with $\hat{K}$. When we set $\hat{K}$ large enough, the results are reasonable.}}
\label{fig:k_comparison}
\end{figure*}
}

\newcommand{\figFFHQfew}{
\begin{figure}[t]
\centering
\includegraphics[width=0.6\columnwidth]{TUNIT_fig4.jpg}
\caption{\small{\textbf{Cross-domain attribute translation using 0.1\% of labeled samples.} As a practical application, we also apply TUNIT to FFHQ with few labels as a form of cross-domain translation. For each attribute, we train TUNIT separately (there are four models.). To this end, we manually label 35 images for each domain -- one contains the attribute and another does not contain it. Then, we train TUNIT with 70 labeled samples (0.1\% of the dataset) and remaining unlabeled samples. To add or remove the attribute, we use the average style vector of each domain. This result shows that TUNIT can greatly reduce the labeling cost.}}
\label{fig:ffhqfew}
\vspace{-0.6cm}
\end{figure}
}


% \newcommand{\figUnlabeled}{
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{figures/section4/TUNITFig4tmp.pdf}
% \caption{\small{Reference-guided image translation results on unlabeled datasets. \textbf{TMPTMPTMP}}}
% \label{fig:unlabeled_reference_guided}
% \vspace{-0.3cm}
% \end{figure*}
% }

\newcommand{\figUnlabeled}{
% 15 / 1.5 / 2.0
\renewcommand{\h}{13.3mm}
\newcommand{\hsrc}{1.33mm}
\newcommand{\hdataset}{1.78mm}
\begin{figure*}[t]
\centering
\hspace{1mm}
\makebox[\h][c]{Source}\hspace{4mm}
\makebox[\h][c]{Reference}\hspace{5mm}
\makebox[\h][c]{FUNIT}\hspace{3mm}
\makebox[\h][c]{TUNIT}\hspace{10mm}
\makebox[\h][c]{Source}\hspace{3mm}
\makebox[\h][c]{Reference}\hspace{5mm}
\makebox[\h][c]{FUNIT}\hspace{3mm}
\makebox[\h][c]{TUNIT}\hspace{0mm}
\vspace{0.5mm}
\\
\rotatebox{90}{\makebox[52mm][c]{\textsc{afhq cat}}}\vspace{1mm}\hspace{0.5mm}
\includegraphics[width=0.2\textwidth]{afhq_cat_input.jpg}\hspace{\hsrc}
\includegraphics[width=0.2\textwidth]{afhq_cat_output.jpg}\hspace{\hdataset}
\rotatebox{90}{\makebox[52mm][c]{\textsc{ffhq}}}\vspace{0mm}
\includegraphics[width=0.2\textwidth]{ffhq_total_input.png}\hspace{\hsrc}
\includegraphics[width=0.2\textwidth]{ffhq_total_output.png}
\vspace{-1.2mm}
\\
\rotatebox{90}{\makebox[52mm][c]{\textsc{afhq wild}}}\vspace{1mm}\hspace{0.5mm}
\includegraphics[width=0.2\textwidth]{afhq_wild_input.jpg}\hspace{\hsrc}
\includegraphics[width=0.2\textwidth]{afhq_wild_output.jpg}\hspace{\hdataset}
\rotatebox{90}{\makebox[52mm][c]{\textsc{lsun car}}}\vspace{0mm}\hspace{0.5mm}
\includegraphics[width=0.2\textwidth]{lsun_input.jpg}\hspace{\hsrc}
\includegraphics[width=0.2\textwidth]{lsun_output.jpg}
\vspace{-0.4cm}
\caption{\small{Reference-guided image translation results on unlabeled datasets.}}
\label{fig:unlabeled_reference_guided}
\vspace{-0.5cm}
\end{figure*}
}

% \newcommand{\figtsnecompare}{
% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.8\textwidth]{figures/section4/unlabeled/tsne/t-sne_bkj.pdf}

% \makebox[0.45\textwidth][c]{\small{(a) t-SNE visualization of FUNIT (left) and TUNIT (right)}}
% \makebox[0.2\textwidth][r]{\small{(b) Representative images}}\hfill

% \caption{t-SNE visualization of our style space trained on AFHQ Wild. Since AFHQ Wild does not have ground-truth labels, each point is colored with the guiding network's prediction. Although we set the number of domains to be larger ($\hat{K}=10$) than it seems to have, the network model practically creates six clusters by closely locating different clusters of one species. 
% % separates one species into two domains, which are so closely located that the model creates six clusters.
% }
% \label{fig:tsne_compare}
% \vspace{-0.4cm}
% \end{figure*}
% }

\newcommand{\figtsnecompare}{
\begin{figure}[t!]
\centering
\includegraphics[width=1.0\columnwidth]{t-sne_new.jpg}

\makebox[0.68\columnwidth][c]{\small{(a) t-SNE of FUNIT (L) / TUNIT (R)}}
\makebox[0.31\columnwidth][l]{\small{(b) Example images}}\hfill
\caption{t-SNE visualization of style space trained on AFHQ Wild. Since AFHQ Wild does not have ground-truth labels, each point is colored with the guiding network's prediction. Although we set the number of domains to be larger ($\hat{K}=10$) than it seems to have, the network practically creates six clusters by closely locating clusters of one species. 
}
\label{fig:tsne_compare}
\vspace{-0.4cm}
\end{figure}
}

\newcommand{\figQualCompare}{
\begin{figure}[t!]
\includegraphics[width=0.495\textwidth]{figures/section4/comparison_animalfaces_new2.pdf}
\includegraphics[width=0.495\textwidth]{figures/section4/comparison_food_new.pdf}\\
\makebox[0.495\linewidth][c]{\footnotesize{(a) AnimalFaces-10}}\hfill
\makebox[0.495\linewidth][c]{(b) Food-10}\hfill

\caption{\textbf{Translation results for the qualitative comparison.} The text next to each row is the same name of the model in \Tref{tab:main}.}
\label{fig:qualitative_compare}
\vspace{-0.3cm}
\end{figure}
}

\newcommand{\figKablation}{
\begin{figure}[t!]
\includegraphics[width=0.99\textwidth]{figures/section4/K_ablation_new_4.pdf}
\caption{\textbf{Robustness against number of clusters, $\hat{K}$.} The performance varies but it mostly works with various $\hat{K}$s.}
\label{fig:k_ablation}
\vspace{-0.5cm}
\end{figure}
}

\newcommand{\figTSNE}{
\begin{figure}[t!]
\includegraphics[width=0.99\textwidth]{figures/section4/t-sne_new_3.pdf}
\caption{\textbf{t-SNE visualization of the style space} of our guiding network trained on AFHQ Wild. Since AFHQ Wild does not have ground-truth labels, each point is colored with guiding network's prediction. Although we set the number of domains to be quite large ($\hat{K}=10$), the network separates one species into two domains, which are so closely located that the model creates six clusters.}
\label{fig:tsne_afhq}
\vspace{-0.5cm}
\end{figure}
}

\newcommand{\figUnsup}{
\begin{figure}[t!]
\includegraphics[width=0.495\textwidth]{figures/section4/unsupervised_cat_half.pdf}
\includegraphics[width=0.495\textwidth]{figures/section4/unsupervised_wild_half.pdf}\\
\makebox[0.495\linewidth][c]{\footnotesize{(a) AFHQ Cat}}\hfill
\makebox[0.495\linewidth][c]{(b) AFHQ Wild}\hfill
\includegraphics[width=0.495\textwidth]{figures/section4/unsupervised_car_half.pdf}
\includegraphics[width=0.495\textwidth]{figures/section4/unsupervised_ffhq_half.pdf}\\
\makebox[0.495\linewidth][c]{\footnotesize{(c) LSUN Cars}}\hfill
\makebox[0.495\linewidth][c]{(d) FFHQ}\hfill
\vspace{-0.2cm}
\caption{\textbf{Unsupervised image-to-image translation examples.} The first row of each image shows the four example images in each domain. Each image is generated with the source image and the average style code of all test images in each cluster.}
\label{fig:unsupervised}
\vspace{-0.3cm}
\end{figure}
}

%%%%%%%%%%%%
% Appendix %
%%%%%%%%%%%%

\newcommand{\figTsneAfhqCat}{
\begin{figure}[!h]
\centering
\vspace{-10mm}
\includegraphics[width=0.96\linewidth]{tsne_afhq_cat.jpg}
\vspace{-10mm}
\caption{\textbf{t-SNE visualization and representative images of each domain for AFHQ Cat.}}
\label{fig:tsne_afhq_cat}
\end{figure}
}

\newcommand{\figTsneAfhqDog}{
\begin{figure}[!h]
\centering
% \vspace{-10mm}
\vspace{1.13cm}
\includegraphics[width=0.96\linewidth]{tsne_afhq_dog.jpg}
\vspace{-10mm}
\caption{\textbf{t-SNE visualization and representative images of each domain for AFHQ Dog.}}
\label{fig:tsne_afhq_dog}
\end{figure}
}

\newcommand{\figTsneFfhq}{
\begin{figure}[!h]
\centering
\vspace{-10mm}
\includegraphics[width=0.96\linewidth]{tsne_ffhq.jpg}
\vspace{-10mm}
\caption{\textbf{t-SNE visualization and representative images of each domain for FFHQ.}}
\label{fig:tsne_ffhq}
\end{figure}
}

\newcommand{\figTsneLsun}{
\begin{figure}[!h]
\centering
\vspace{-10mm}
\includegraphics[width=0.96\linewidth]{tsne_lsun.jpg}
\vspace{-10mm}
\caption{\textbf{t-SNE visualization and representative images of each domain for LSUN Car.}}
\label{fig:tsne_lsun}
\end{figure}
}

\newcommand{\figAppAnimalFaces}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\linewidth]{app_animal_avg.JPG}\\
\makebox[0.8\linewidth][c]{\textbf{(a) Results guided by average style vectors}}\vspace{1mm}
\includegraphics[width=0.75\linewidth]{app_animal_ref.JPG}\\
\makebox[0.8\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-3mm}
\caption{AnimalFaces-10, unsupervised image-to-image translation results.}
\label{fig:AppAnimalFaces}
\end{figure*}
}

\newcommand{\figAppAFHQCat}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\textwidth]{app_cat_avg.JPG}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.75\textwidth]{app_cat_ref.JPG}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{AFHQ Cat, unsupervised image-to-image translation results.}
\label{fig:AppAFHQCat}
\end{figure*}
}

\newcommand{\figAppAFHQDog}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\textwidth]{app_dog_avg.JPG}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.75\textwidth]{app_dog_ref.JPG}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{AFHQ Dogs, unsupervised image-to-image translation results.}
\label{fig:AppAFHQDog}
\end{figure*}
}

\newcommand{\figAppAFHQWild}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\textwidth]{app_wild_avg.JPG}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.75\textwidth]{app_wild_ref.JPG}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{AFHQ Wild, unsupervised image-to-image translation results.}
\label{fig:AppAFHQWild}
\end{figure*}
}

\newcommand{\figAppFFHQ}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\textwidth]{app_ffhq_avg.JPG}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.75\textwidth]{app_ffhq_ref.JPG}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{FFHQ, unsupervised image-to-image translation results.}
\label{fig:AppFFHQ}
\end{figure*}
}

\newcommand{\figAppLSUN}{
\begin{figure*}[b]
\centering
\vspace{-7mm}
\includegraphics[width=0.75\textwidth]{app_lsun_avg.JPG}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.75\textwidth]{app_lsun_ref.JPG}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{LSUN Car, unsupervised image-to-image translation results.}
\label{fig:AppLSUN}
\end{figure*}
}

\newcommand{\figAppCatVsFUNIT}{
\begin{figure}[!h]
\centering
\includegraphics[width=0.98\columnwidth]{app_afhq_cat_appendix_vs_funit.JPG}\\
\caption{AFHQ Cat, unsupervised reference-guided image-to-image translation results of FUNIT and TUNIT. The content and the style are from the source and the reference, respectively. While FUNIT usually fails to reflect the style of the reference image, TUNIT generates the fake images with the style -- color, fur texture.}
\label{fig:AppCatVsFUNIT}
\end{figure}
}

\newcommand{\figAppWildVsFUNIT}{
\begin{figure}[!h]
\centering
\includegraphics[width=0.98\columnwidth]{app_afhq_wild_appendix_vs_funit.JPG}\\
\caption{AFHQ Wild, unsupervised reference-guided image-to-image translation results of FUNIT and TUNIT. FUNIT rarely reflects the correct style of the reference image -- the species, on the other hand, TUNIT translates the source image to the correct species.}
\label{fig:AppWildVsFUNIT}
\end{figure}
}

\newcommand{\figAppLSUNVsFUNIT}{
\begin{figure}[!h]
\centering
\vspace{1.555cm}
\includegraphics[width=0.98\columnwidth]{app_lsun_appendix_vs_funit.JPG}\\
\caption{LSUN Car, unsupervised reference-guided image-to-image translation results of FUNIT and TUNIT. While TUNIT generates plausible and changes the color of the source image to that of the reference image, FUNIT not also generates unrealistic image but also fails to changes the color.}
\label{fig:AppLSUNVsFUNIT}
\end{figure}
}

\newcommand{\figAppFFHQVsFUNIT}{
\begin{figure}[!h]
\centering
\includegraphics[width=0.98\columnwidth]{app_ffhq_appendix_vs_funit.JPG}\\
\caption{FFHQ, unsupervised reference-guided image-to-image translation results of FUNIT and TUNIT. Our model, TUNIT can remove or add the glasses to the source while preserving the identity better than FUNIT. In addition, TUNIT can change the hair color (last column) and the hair style -- especially, bang (fifth column). It is hard to specify the definition of domains in the results of FUNIT while domains of TUNIT are more interpretable.}
\label{fig:AppFFHQVsFUNIT}
\end{figure}
}


\newcommand{\figAppStoW}{
\begin{figure*}[b]
\centering
\vspace{-7mm} 
\includegraphics[width=0.85\textwidth]{app_summer2winter_avg.jpg}\\
\makebox[1\linewidth][c]{\textbf{(a) Results guided by the average style code of each domain}}\vspace{1mm}
\includegraphics[width=0.85\textwidth]{app_summer2winter_ref.jpg}\\
\makebox[1\linewidth][c]{\textbf{(b) Results guided by reference images}}
\vspace{-5mm}
\caption{Summer2Winter (S2W), unsupervised image-to-image translation results.}
\label{fig:AppStoW} 
\end{figure*}
}

\newcommand{\figAppPtoU}{
\begin{figure*}[b]
\centering
\vspace{-7mm} 
\includegraphics[width=0.85\textwidth]{app_photo2ukiyoe_ref.jpg}\\
\makebox[1\linewidth][c]{\textbf{Results guided by reference images}}
\vspace{-5mm}
\caption{Photo2Ukiyoe, unsupervised image-to-image translation results.}
\label{fig:AppPtoU} 
\end{figure*}
}

\newcommand{\figAppSEMIT}{
\begin{figure*}[b]
\centering
\vspace{-7mm} 
\includegraphics[width=0.85\textwidth]{vsSEMIT.jpg}\\
% \makebox[1\linewidth][c]{\textbf{Results guided by reference images}}
\caption{Qualitative comparison with SEMIT and FUNIT, semi-supervised translation results on AnimalFaces-149 (1\% of labeled samples are used).}
\label{fig:AppSEMIT} 
\end{figure*}
}

\newcommand{\figAppLPIPS}{
\begin{figure*}[b]
\centering
\includegraphics[width=1\textwidth]{lpips_vs_fid_fig.pdf}\\
\vspace{-5mm}
\caption{\textbf{LPIPS and FID of models and their status.}}
\label{fig:AppLPIPS} 
\end{figure*}
}



==> Truly unsupervised img2img (arXiv version)/table.tex <==
\newcommand{\tabmain}{
\begin{table*}[t]
\centering
\newcolumntype{x}{>{\centering\arraybackslash\hspace{0pt}}p{17mm}}
\newcolumntype{s}{>{\centering\arraybackslash\hspace{0pt}}p{6mm}}
\small{
\begin{tabular}{|l@{\hspace{2.5mm}}l|p{6mm}p{17mm}p{6mm}|p{6mm}p{17mm}p{6mm}|}
\hline
& \multirow{2}{*}{\textbf{Configuration}}
    & \multicolumn{3}{c|}{\textbf{AnimalFaces-10}}
    & \multicolumn{3}{c|}{\textbf{Food-10}}
\\
&
    & mFID & \makebox[17mm][c]{D \& C} & Acc.
    & mFID & \makebox[17mm][c]{D \& C} & Acc.
\\ \hline
\\[-0.8em]
\arch{a} & Baseline FUNIT  (supervised)\ \                   %
    & 74.0          & 0.749 / 0.671   & \textbf{1.000}         %
    & 68.4          & 0.989 / 0.782   & \textbf{1.000}         %
\\[0.3mm]
\arch{b} & (\arch{a}) + Improved G \& D (supervised) \ \                                 %
    & \textbf{46.2}          & \textbf{0.896}  / \textbf{0.732}         & \textbf{1.000}         %
    & \textbf{57.6}          & \textbf{1.284} / \textbf{0.857}         & \textbf{1.000}         %
\\[0.3mm] \hline
\\[-0.8em]
\arch{c} & (\arch{b}) + K-means on image space\ \                                 %
    & 110.7         & 0.822  / 0.615         & 0.215         %
    & 90.7          & 0.849 / 0.648         & 0.201         %
\\[0.3mm]
\arch{d} & (\arch{b}) + K-means on feature space\ \                          %
    & 76.2          & 0.770 / 0.597         & 0.428         %
    & 64.6          & 0.968 / 0.808         & 0.331         %
\\[0.3mm]
\arch{e} & (\arch{b}) + Differentiable clustering\ \                        %
    & 73.5          & 0.940 / 0.588         & 0.680         %
    & 64.2          & 1.038 / 0.819         & 0.542         %
\\[0.3mm]
% \hline
%\\[-0.8em]
\arch{f} & TUNIT w/ sequential training\ \                                      %
    & \textbf{46.0}    & 1.060 / 0.789         & \textbf{0.850}   %
    & 61.1    & 0.908 / 0.777         & \textbf{0.860}   %
\\[0.3mm]
\arch{g} & TUNIT w/ joint training\ \                                      %
    & 47.7    & \textbf{1.039} / \textbf{0.805}         & 0.841   %
    & \textbf{52.2}    & \textbf{1.079} / \textbf{0.875}         & 0.848   %
\\[0.3mm] \hline
\end{tabular}\vspace{0mm}}
\caption{\small{
Comparison results. mFID, Density / Coverage (D\&C), and classification accuracy (Acc) of each training configuration. Note that the configurations (\arch{a}) - (\arch{b}) use ground-truth class labels, while (\arch{c}) - (\arch{g}) use pseudo-labels. We \textbf{bold} the best results separately for supervised and unsupervised settings. For D\& C, we boldify the one which has the best coverage that has a clear maximum.}
}\vspace{-3mm}
\label{tab:main}
\end{table*}
}

%%% 임시
% \makebox[0.67\linewidth][c]{\footnotesize{(a) t-SNE visualization of FUNIT (left) and TUNIT (right)}}\hfill
% \makebox[0.33\linewidth][c]{(b) Representative images}\hfill
\newcommand{\tabKcomparisonn}{
\begin{table}[t]
\centering
\begin{minipage}[]{0.4\columnwidth}
    \centering
    % \vspace{-2mm}
    \includegraphics[keepaspectratio=false, width=1.0\linewidth,height=1.0\linewidth]{tunit_train_animal_k10_noticks.png}
    \footnotesize{(a) t-SNE of $\hat{K}$=10}
\end{minipage}\quad
\begin{minipage}[]{0.4\columnwidth}
    \centering
    % \vspace{-2mm}    
    \includegraphics[keepaspectratio=false, width=1.0\linewidth,height=1.0\linewidth]{tunit_train_animal_k20_noticks.png}
    \footnotesize{(b) t-SNE of $\hat{K}$=20}
\end{minipage}\quad

\begin{minipage}[]{0.9\columnwidth}
    \centering
    \footnotesize{
    \begin{tabular}{|l@{\hspace{1.0mm}}l|p{5mm}p{17mm}|p{5mm}p{17mm}|}
    \hline
    & \multirow{2}{*}{\textbf{$\hat{K}$}}
        & \multicolumn{2}{c|}{\textbf{AnimalFaces-10}}
        & \multicolumn{2}{c|}{\textbf{Food-10}}
    \\ 
    &
        & \makebox[6mm][c]{mFID} & \makebox[17mm][c]{D \& C}
        & \makebox[6mm][c]{mFID} & \makebox[17mm][c]{D \& C}
    \\ \hline
    \\[-0.8em]
    & \footnotesize{$1$} \ \              
        & 129.6          & 0.561 / 0.512        
        & 95.1              & 1.113 / 0.771        
    \\[0.3mm]
    & \footnotesize{$4$} \ \ 
        & 77.7          & 0.879 / 0.738        
        & 67.4             & 0.851 / 0.785        
    \\[0.3mm]
    & \footnotesize{$7$} \ \  
        & 62.7         & 1.016 / 0.729
        & 52.7            & 1.024 / 0.846 
    \\[0.3mm]
    & \footnotesize{$10$} \ \  
        & \textbf{47.7}          & \textbf{1.039} / \textbf{0.805} 
        & \textbf{52.2}             & \textbf{1.079} / \textbf{0.875}         %
    \\[0.3mm]
    & \footnotesize{$13$}\ \   
        & 56.8          & 0.993 / 0.720  
        & 54.8             & 0.970 / 0.845         
    \\[0.3mm]
    & \footnotesize{$16$}\ \  
        & 54.1           & 1.093 / 0.782   
        & 54.8              & 1.029 / 0.857       
    \\[0.3mm]
    & \footnotesize{$20$}\ \  
        & 55.4           & 1.019 / 0.778   
        & 57.7              & 0.937 / 0.846     
    \\[0.3mm] 
     & \footnotesize{$50$}\ \  
    & 63.8           & 0.858 / 0.701
    & 60.8              & 1.067 / 0.837
\\[0.3mm]
 & \footnotesize{$500$}\ \  
    & 67.2           & 0.921 / 0.694
    & 63.2              & 0.986 / 0.826
\\[0.3mm]
 & \footnotesize{$1000$}\ \  
    & 66.9           & 0.908 / 0.707
    & 60.7              & 0.945 / 0.845
\\[0.3mm]
    
    \hline
\end{tabular}}
% \footnotesize{(c)}
\end{minipage}
% \vspace{0mm}
\caption{
\small{t-SNE visualization of the model with (a) $\hat{K}$=10 and (b) $\hat{K}$=20 trained on AnimalFaces-10 and quantitative evaluation of our method by varying the number of pseudo domains $\hat{K}$. Each point is colored with the ground-truth labels. As shown in t-SNE visualizations, even if $\hat{K}$ is set to overly larger than the actual number of domains, the guiding network clusters the domains reasonably well. For D\& C, we bold the one which has the best coverage that has a clear maximum.}
}
\vspace{-5mm}
\label{tab:k_comparison}
\end{table}
}
%%%%임시

\newcommand{\tabKcomparison}{
\begin{table}[t]
\centering
\begin{minipage}[]{0.35\linewidth}
    \centering
    \vspace{-2mm}
    \includegraphics[width=1.0\linewidth]{figures/section4/k_comparison/tunit_train_animal_k20.png}

\end{minipage}\quad
\begin{minipage}[]{0.6\linewidth}
    \centering
    \footnotesize{
    \begin{tabular}{|l@{\hspace{1.0mm}}l|p{6mm}p{17mm}|p{6mm}p{17mm}|}
    \hline
    & \multirow{2}{*}{\textbf{$\hat{K}$}}
        & \multicolumn{2}{c|}{\textbf{AnimalFaces-10}}
        & \multicolumn{2}{c|}{\textbf{Food-10}}
    \\ 
    &
        & \makebox[6mm][c]{mFID} & \makebox[17mm][c]{D \& C}
        & \makebox[6mm][c]{mFID} & \makebox[17mm][c]{D \& C}
    \\ \hline
    \\[-0.8em]
    & \footnotesize{$1$} \ \              
        & 129.6          & 0.561 / 0.512        
        & 95.1              & \textbf{1.113} / 0.771        
    \\[0.3mm]
    & \footnotesize{$4$} \ \ 
        & 77.7          & 0.879 / 0.738        
        & 67.4             & 0.851 / 0.785        
    \\[0.3mm]
    & \footnotesize{$7$} \ \  
        & 62.7         & 1.016 / 0.729
        & 52.7            & 1.079 / \textbf{0.875} 
    \\[0.3mm]
    & \footnotesize{$10$} \ \  
        & \textbf{47.7}          & 1.039 / \textbf{0.805} 
        & \textbf{52.2}             & 1.079 / \textbf{0.875}         %
    \\[0.3mm]
    & \footnotesize{$13$}\ \   
        & 56.8          & 0.993 / \textbf{0.805}  
        & 54.8             & 0.970 / 0.845         
    \\[0.3mm]
    & \footnotesize{$16$}\ \  
        & 54.1           & \textbf{1.093} / 0.782   
        & 54.8              & 1.029 / 0.857       
    \\[0.3mm]
    & \footnotesize{$20$}\ \  
        & 55.4           & 1.019 / 0.778   
        & 57.7              & 0.937 / 0.846     
    \\[0.3mm] 
    \hline
\end{tabular}}
\end{minipage}
\vspace{0mm}\caption{
\small{t-SNE visualization of the model with $\hat{K}$=20 trained on AnimalFaces-10 and quantitative evaluation of our method by varying the number of pseudo domains $\hat{K}$. The qualitative results can be seen in \Fref{fig:k_comparison}.}
}\vspace{-2mm}
\label{tab:k_comparison}
\end{table}
}

% old without t-sne
\iffalse
\newcommand{\tabKcomparison}{
\newcommand{\hrow}{13.5mm}
\begin{table*}[t]
\centering
\newcolumntype{x}{>{\centering\arraybackslash\hspace{0pt}}p{\hrow}}
\footnotesize{
\begin{tabular}{|l@{\hspace{2.5mm}}l|xxx|xxx|}
\hline
& \multirow{2}{*}{\textbf{Configuration}}
    & \multicolumn{3}{c|}{\textbf{AnimalFaces-10}}
    & \multicolumn{3}{c|}{\textbf{Food-10}}
\\
&
    & \makebox[\hrow][c]{mFID} & \makebox[\hrow][c]{Density} & \makebox[\hrow][c]{Coverage}
    & \makebox[\hrow][c]{mFID} & \makebox[\hrow][c]{Density} & \makebox[\hrow][c]{Coverage}
\\ \hline
\\[-0.8em]
 & TUNIT (\footnotesize{$K=1$}) \ \              
    & 129.6          & 0.561   & 0.512        
    & 95.1              & \textbf{1.113}       & 0.771        
\\[0.3mm]
 & TUNIT (\footnotesize{$K=4$}) \ \ 
    & 77.7          & 0.879         & 0.738        
    & 67.4             & 0.851              & 0.785        
\\[0.3mm]
 & TUNIT (\footnotesize{$K=7$}) \ \  
    & 62.7         & 1.016         & 0.729
    & 52.7            & 1.079             & \textbf{0.875} 
\\[0.3mm]
 & TUNIT (\footnotesize{$K=10$}) \ \  
    & \textbf{47.7}          & 1.039        & \textbf{0.805} 
    & \textbf{52.2}             & 1.079       & \textbf{0.875}         %
\\[0.3mm]
 & TUNIT (\footnotesize{$K=13$})\ \   
    & 56.8          & 0.993         & \textbf{0.805}  
    & 54.8             & 0.970                      & 0.845         
\\[0.3mm]
 & TUNIT (\footnotesize{$K=16$})\ \  
    & 54.1           & \textbf{1.093}           & 0.782   
    & 54.8              & 1.029               & 0.857       
\\[0.3mm]
 & TUNIT (\footnotesize{$K=20$})\ \  
    & 55.4           & 1.019         & 0.778   
    & 57.7              & 0.937             & 0.846     
\\[0.3mm]
 & TUNIT (\footnotesize{$K=50$})\ \  
    & 63.8           & 0.858         & 0.701   
    & 65.6              & 0.894             & 0.796     
\\[0.3mm]
 & TUNIT (\footnotesize{$K=500$})\ \  
    & 67.2           & 0.921         & 0.694   
    & 67.1              & 0.874             & 0.786     
\\[0.3mm]
 & TUNIT (\footnotesize{$K=1000$})\ \  
    & 66.9           & 0.908         & 0.707   
    & 66.3              & 0.909             & 0.773     
\\[0.3mm]\hline
\end{tabular}\vspace{0mm}}
\caption{
\small{Quantitative evaluation of our method by varying the number of pseudo domains $\hat{K}$. The qualitative results can be seen in \Fref{fig:k_comparison}.}
}\vspace{-2mm}
\label{tab:k_comparison}
\end{table*}
}
\fi

\newcommand{\tabsemi}{
\newcommand{\hrow}{5mm}
\begin{table*}[t]
\centering
\newcolumntype{x}{>{\centering\arraybackslash\hspace{-2mm}}p{\hrow}}
\footnotesize{
\begin{tabular}{|l@{\hspace{1mm}}l|xxxx|xxxx|xxxx|xxxx|}
\hline
% & \multirow{2}{*}{\textbf{Configuration}}
& \multirow{2}{*}{\textbf{Model}}
    & \multicolumn{8}{c|}{\textbf{AnimalFaces-10}}
    & \multicolumn{8}{c|}{\textbf{Food-10}}
\\
&
 & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
 & \makebox[\hrow][c]{20\%} & \makebox[\hrow][c]{40\%} & \makebox[\hrow][c]{60\%} & \makebox[\hrow][c]{80\%}
 & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
 & \makebox[\hrow][c]{20\%} & \makebox[\hrow][c]{40\%} & \makebox[\hrow][c]{60\%} & \makebox[\hrow][c]{80\%}
\\ \hline
\\[-0.8em]
& FUNIT~\cite{2019FUNIT} \ \                   %
    & 179.8    & 174.3     & 154.3   & 144.0      %
    & 124.4    & 106.4     & 96.0   & 79.6      %
    & 195.7     & 159.2      & 141.2  & 135.2               %
    & 111.4     & 85.8      & 74.8  & 70.3               %
\\[0.3mm]
& SEMIT~\cite{wang2020semit} \ \                   %
    & 68.9    & 63.0     & 63.5   & 60.3      %
    & 57.3    & 64.3     & 66.1   & 62.8      %
    & 70.7     & 66.7      & 65.3  & 65.1               %
    & 65.2     & 62.8      & 61.6  & 64.1               %
\\[0.3mm]
& TUNIT (ours)\ \                        
    & \textbf{42.0}    & \textbf{42.6}     & \textbf{43.9}   & \textbf{46.2}               %
    & \textbf{42.0}    & \textbf{42.6}     & \textbf{43.9}   & \textbf{46.2}               %
    & \textbf{53.6}     & \textbf{56.2}      & \textbf{52.8} & \textbf{53.4}                %
    & \textbf{53.6}     & \textbf{56.2}      & \textbf{52.8} & \textbf{53.4}                %
\\[0.3mm] \hline

& \multirow{2}{*}{\textbf{Model}}
    & \multicolumn{8}{c|}{\textbf{AnimalFaces-149}}
    & \multicolumn{8}{c|}{\textbf{Food-101}}
\\
&
 & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
 & \makebox[\hrow][c]{20\%} & \makebox[\hrow][c]{40\%} & \makebox[\hrow][c]{60\%} & \makebox[\hrow][c]{80\%}
 & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
 & \makebox[\hrow][c]{20\%} & \makebox[\hrow][c]{40\%} & \makebox[\hrow][c]{60\%} & \makebox[\hrow][c]{80\%}
\\ \hline
\\[-0.8em]
& FUNIT~\cite{2019FUNIT} \ \                   %
    & 147.3    & 133.6     & 116.9   & 101.7      %
    & 102.7    & 112.4     & 102.9   & 100.3      %
    & 136.8    & 94.9     & 80.9   & 72.6               %
    & 67.6    & 66.5     & \textbf{66.4}   & 67.4               %
\\[0.3mm]
& SEMIT~\cite{wang2020semit} \ \                   %
    & 137.9    & 123.1     & 134.0   & 120.3      %
    & 113.5    & 114.5     & 116.9   & 116.6      %
    & \textbf{74.7}    & 81.7     & \textbf{71.2}   & \textbf{72.5}               %
    & 68.4    & 68.7     & 69.8   & 69.5               %
\\[0.3mm]
& TUNIT (ours)\ \                        
    & \textbf{104.9}    & \textbf{99.9}     & \textbf{96.8}   & \textbf{87.5}      %
    & \textbf{84.0}    & \textbf{79.9}     & \textbf{80.1}   & \textbf{78.4}      %
    & 75.0    & \textbf{74.4}     & 74.9   & 75.2               %
    & \textbf{64.7}    & \textbf{64.0}     & 68.2   & \textbf{66.8}               %
\\[0.3mm] \hline

\end{tabular}\vspace{-2mm}
}
\caption{
\small{Quantitative evaluation (mFID) when few labels are available during training. We note that TUNIT is the same as \texttt{G} in \Tref{tab:main}}
}\vspace{-3mm}
\label{tab:semi_wo_cls}
\end{table*}
}

% \newcommand{\tabsemicls}{
% \begin{table*}[t]
% \centering
% \newcolumntype{x}{>{\centering\arraybackslash\hspace{0pt}}p{\hrow}}
% \footnotesize{
% \begin{tabular}{|l@{\hspace{2.5mm}}l|xxxx|xxxx|}
% \hline
% & \multirow{2}{*}{\textbf{Configuration}}
%     & \multicolumn{4}{c|}{\textbf{AnimalFaces-10}}
%     & \multicolumn{4}{c|}{\textbf{Food-10}}
% \\
% &
%  & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
%  & \makebox[\hrow][c]{1\%} & \makebox[\hrow][c]{2\%} & \makebox[\hrow][c]{4\%} & \makebox[\hrow][c]{8\%}
% \\ \hline
% \\[-0.8em]
% \arch{a} & FUNIT \ \                   %
%     & 107.8    & 104.7     & 90.3   & 93.9      %
%     & 71.9     & 71.5      & 71.6  & 69.0               %
% \\[0.3mm]

% \arch{g} & TUNIT (ours) \ \                        
%     & \textbf{47.9}    & \textbf{44.8}     & \textbf{42.7}   & \textbf{42.4}               %
%     & \textbf{54.5}     & \textbf{56.1}      & \textbf{55.9} & \textbf{55.8}                %
% \\[0.3mm] \hline
% \end{tabular}\vspace{-2mm}}
% \caption{
% Quantitative evaluation (mFID) when few labels are available during training. Here, an auxliary classifier is adopted to improve the FUNIT baseline by giving pseudo-labels to $\mathcal{D}_{un}$. 
% }
% % \vspace{-5.5mm}
% \label{tab:semi_w_cls}
% \end{table*}
% }


\newcommand{\tableModel}{
\begin{table}[t!]
    \centering
    \caption{\small{\textbf{Density, Coverage, mFID and Accuracy of each model.} The lower mFID and the closer Density and Coverage to 1.0, the better model.}}
    \resizebox{\columnwidth}{!}{
    {
    \begin{tabular}{| c ||c | l | c | c c c | c|}
            \hline
            Dataset & Tag & \multicolumn{1}{c|}{Translation and Clustering} & Step & mFID & Density & Coverage & Label accuracy \\
            \hline
            \multirow{8}{*}{AnimalFaces-10}& A & FUNIT + Supervised & 1 & 74.0 & 0.749 & 0.671 & 100\% \\
            & B & FUNIT + Our arch + Supervised & 1 & 46.2 & 0.896 & 0.732 & 100\% \\
            \cline{2-8}
            & C & FUNIT + Our arch + K-Means (flatten image) & 2 & 110.7 & 0.822 & 0.615 & 21.5\%\\
            % & D & FUNIT + Our arch + K-Means (random feature) & 2 & 132.1 & 0.732 & 0.598 & 15.5\%\\
            & D & FUNIT + Our arch + K-Means (MoCo v2 pretraining) & 3 & 76.2 & 0.770 & 0.597 & 42.8\%\\
            & E & FUNIT + Our arch + Differentiable Clustering & 2 & 73.5 & 0.940 & 0.588 & 68.0\%\\
            & F & FUNIT + Our arch + MoCo + Differentiable Clustering & 2 & 59.1 & 1.075 & 0.703 & \textbf{85.0\%}\\
            & G & TUNIT (2 step) & 2 & \textbf{46.0} & 1.060 & 0.789 & 84.1\%\\
            & H & TUNIT & 1 & 47.7 & \textbf{1.039} & \textbf{0.805} & 84.1\%\\
            \hline
            \hline
            \multirow{8}{*}{Food-10} & A & FUNIT + Supervised & 1 & 68.4 & \textbf{0.989} & 0.782 & 100\% \\
            & B & FUNIT + Our arch + Supervised & 1 & 57.6 & 1.284 & 0.857 & 100\% \\
            \cline{2-8}
            & C & FUNIT + Our arch + K-Means (flatten image) & 2 & 90.7 & 0.849 & 0.648 & 20.1\%\\
            % & D & FUNIT + Our arch + K-Means (random feature) & 2 & 100.4 & 0.913 & 0.679 & 17.1\%\\
            & D & FUNIT + Our arch + K-Means (MoCo v2 pretraining) & 3 & 64.6 & 0.968 & 0.808 & 33.1\%\\
            & E & FUNIT + Our arch + Differentiable Clustering & 2 & 64.2 & 1.038 & 0.819 & 54.2\%\\
            & F & FUNIT + Our arch + MoCo + Differentiable Clustering & 2 & 56.3 & 1.201 & 0.857 & \textbf{86.0\%}\\
            & G & TUNIT (2 step) & 2 & 61.1 & 0.908 & 0.777 & 84.8\%\\
            & H & TUNIT & 1 & \textbf{52.2} & 1.080 & \textbf{0.874} & 84.8\%\\
            \hline
    \end{tabular}
    }}
  \label{table:modelCompare}
\end{table}
}

% \newcommand{\tableRatio}{
% \begin{table}[t!]
%     \centering
%     \caption{\textbf{Comparison TUNIT with FUNIT when few labels are available.} The value is mFID. ``Without Classifier'': Training FUNIT without classifier. ``With Classifier'': FUNIT with classifier.}
%     \resizebox{0.9\columnwidth}{!}{
%     {
%     \begin{tabular}{| c| c || c | c | c | c | c| c| c|}
%             \hline
%             Scheme & Dataset & Model & 0\% & 20\% & 40\% & 60\% & 80\% & 100\% \\
%             \hline
%             \multirow{4}{*}{{\makecell{Without \\ Classifier}}} & \multirow{2}{*}{AnimalFaces-10} & FUNIT & - & 124.4 & 106.4 & 96.0 & 79.6 & 74.0 \\
%             & & TUNIT & 47.7 & 42.0 & 42.6 & 43.9 & 46.2 & 45.5 \\
%             \cline{2-9}
%             & \multirow{2}{*}{Food-10} & FUNIT & - & 111.4 & 85.8 & 74.8 & 70.3 & 68.2 \\
%             & & TUNIT & 52.2 & 53.6 & 56.2 & 52.8 & 53.4 & 58.4 \\
%             \hline
%             \hline
%             Scheme & Dataset & Model & 1\% & \ \ 2\% & \ \ 4\% & \ \ 6\% & \ \ 8\% & \ \ 10\% \\
%             \hline
%             \multirow{4}{*}{{\makecell{With \\ Classifier}}} & \multirow{2}{*}{AnimalFaces-10} & FUNIT & 107.8 & 104.7 & 90.3 & 90.8 & 93.9 & 87.9 \\
%             & & TUNIT & 47.9 & 44.8 & 42.7 & 43.5 & 42.4 & 43.6 \\
%             \cline{2-9}
%             & \multirow{2}{*}{Food-10} & FUNIT & 71.9 & 71.5 & 71.6 & 68.6 & 69.0 & 70.7 \\
%             & & TUNIT & 54.5 & 56.1 & 55.9 & 54.5 & 55.8 & 55.9 \\
%             \hline
%     \end{tabular}
%     }}
%   \label{table:ratioCompare}
%   \vspace{-0.3cm}
% \end{table}
% }

==> abstract.tex <==
% \twocolumn[{
% \renewcommand\twocolumn[1][]{#1}
% \maketitle
% \vspace{-0.7 cm}
% \begin{center}
%     \centering 
%     \vspace{-0.0 cm}
%     \includegraphics[width=1\textwidth]{teaser_3row.pdf}
%     \captionof{figure}{Our model is able to conduct image-to-image translation without any supervision. The output images are generated with the source image and the average style code of each estimated domain. The breed of the output cat changes according to the domain while preserving the pose of the source image.} 
%     \label{fig:teaser}
% \end{center}
% }]
\begin{abstract}
\vspace{-0.3cm}
Every recent image-to-image translation model inherently requires either image-level (\ie input-output pairs) or set-level (\ie domain labels) supervision. However, even set-level supervision can be a severe bottleneck for data collection in practice. In this paper, we tackle image-to-image translation in a fully unsupervised setting, \ie, neither paired images nor domain labels. To this end, we propose a truly unsupervised image-to-image translation model (TUNIT) that simultaneously learns to separate image domains and translates input images into the estimated domains. 
Experimental results show that our model achieves comparable or even better performance than the set-level supervised model trained with full labels, generalizes well on various datasets, and is robust against the choice of hyperparameters (\eg the preset number of pseudo domains). Furthermore, TUNIT can be easily extended to semi-supervised learning with a few labeled data. The source code is available at \url{https://github.com/clovaai/tunit}.
\end{abstract}
\vspace{-0.0 cm}
